MultiActor-Audiobook: Zero-Shot Audiobook Generation with Faces and Voices of Multiple Speakers

We introduce MultiActor-Audiobook, a zero-shot approach for generating audiobooks that automatically produces consistent, expressive, and speaker-appropriate prosody, including intonation and emotion. Previous audiobook systems have several limitations: they require users to manually configure the speaker's prosody, read each sentence with a monotonic tone compared to voice actors, or rely on costly training. However, our MultiActor-Audiobook addresses these issues by introducing two novel processes: (1) MSP (**Multimodal Speaker Persona Generation**) and (2) LSI (**LLM-based Script Instruction Generation**). With these two processes, MultiActor-Audiobook can generate more emotionally expressive audiobooks with a consistent speaker prosody without additional training. We compare our system with commercial products, through human and MLLM evaluations, achieving competitive results. Furthermore, we demonstrate the effectiveness of MSP and LSI through ablation studies.

==> relatedwork.tex <==
\section{Related Work}
\subsection{Emotional TTS System}
    
    
    % (Prompt 없이 그냥 임베딩, 학습, 혹은 제로샷 등으로 emotion 조정)
    % A Neural TTS System with Parallel Prosody Transfer from Unseen Speakers
    % A Discourse-level Multi-scale Prosodic Model for Fine-grained Emotion Analysis
    % PRESENT: Zero-Shot Text-to-Prosody Control
    % E2 TTS: EMBARRASSINGLYEASYFULLYNON-AUTOREGRESSIVEZERO-SHOTTTS
    % VOICECRAFT: Zero-Shot Speech Editing and Text-to-Speech in the Wild
    % Voicebox: Text-Guided Multilingual Universal Speech Generation at Scale
    % TTS System은 발화자의 감정에 따라 억양, 톤, 피치가 달라지는 것이 자연스럽다. 이러한 감정을 조정하는 방식으로는, 화자 임베딩을 학습하는 방법과, 제로샷 컨트롤을 하는 방법이 있다. 
    
    % (Prompt로 emotion 임의 조정 가능)
    % EmoDubber: Towards High Quality and Emotion Controllable Movie Dubbing
    % Facial Expression-Enhanced TTS: Combining Face Representation and Emotion Intensity for Adaptive Speech
    % PROMPT TTS : CONTROL LABLE TEXT-TO-SPEECH WITH TEXT DESCRIPTIONS
    % AudioBox
    % PROMPTTTS 2: DESCRIBING AND GENERATING VOICES WITH TEXT PROMPT
    %  PROMPTTTS++: CONTROLLINGSPEAKERIDENTITYINPROMPT-BASED TEXT-TO-SPEECH USINGNATURALLANGUAGEDESCRIPTIONS
    % TEXTROLSPEECH:ATEXTSTYLECONTROLSPEECHCORPUSWITHCODEC LANGUAGETEXT-TO-SPEECHMODELS
    % DreamVoice: Text-Guided Voice Conversio
    % EmoSpeech: Guiding FastSpeech2 Towards Emotional Text to Speech
    % EXPRESSIVE TTS DRIVEN BY NATURAL LANGUAGE PROMPTS USING FEW HUMAN ANNOTATIONS 
    
    
\subsection{Consistent Voice Synthesis Based on Multimodal Sources}
    % 억양 오디오 SOURCE
    % ComedicSpeech
    % Controlling your Attributes in Voice (나이,성별 등으로 정체성 유지) 
    % YourTTS: Towards Zero-Shot Multi-Speaker TTS and Zero-Shot Voice Conversion for Everyone
    % Transformer-based Multimodal Information Fusion for Facial Expression Analysis(둘 다)
    % VITA-1.5: Towards GPT-4o Level Real-Time Vision and Speech Interaction(둘 다)
    %  MM-TTS:Multi-Modal Prompt Based Style Transfer for Expressive Text-to-Speech Synthesis(둘다)

    
    % 이미지 Source
    % EmotiveTalk: Expressive Talking Head Generation through Audio Information Decoupling and Emotional Video Diffusion
    % Facial Expression-Enhanced TTS: Combining Face Representation and Emotion Intensity for Adaptive Speech
    % Multi-modal Attention for Speech Emotion Recognition
    %  FVTTS: Face Based Voice Synthesis for Text-to-Speech
    % Hear Your Face: Face-based voice conversion with F0 estimation
    % CHATANYTHING: FACETIME CHAT WITH LLM-ENHANCED PERSONAS
    
    %  MM-TTS:Multi-Modal Prompt Based Style Transfer for Expressive Text-to-Speech Synthesis(둘다)
    % FleSpeech: Flexibly Controllable Speech Generation with Various Prompts(둘다)
    % Transformer-based Multimodal Information Fusion for Facial Expression Analysis(둘 다)
    % VITA-1.5: Towards GPT-4o Level Real-Time Vision and Speech Interaction(둘 다)
    

    
\subsection{Audiobook Generation System}
    % From Text to Sound: A Preliminary Study on Retrieving Sound Effects to Radio Stories
    % NarrativePlay: Interactive Narrative Understanding
    % Rule-Based Storytelling Text-to-Speech (TTS) Synthesis
    % Sound of Story: Multi-modal Storytelling with Audio
    % STORY TTS: A HIGHLY EXPRESSIVE TEXT-TO-SPEECH DATASET WITH RICH TEXTUAL EXPRESSIVENESS ANNOTATIONS
